A Meta-learning Framework for Tuning Parameters of Protection Mechanisms in Trustworthy Federated Learning

Trustworthy Federated Learning (TFL) typically leverages protection mechanisms to guarantee privacy. However, protection mechanisms inevitably introduce utility loss or efficiency reduction while protecting data privacy. Therefore, protection mechanisms and their parameters should be carefully chosen to strike an optimal tradeoff between \textit{privacy leakage}, \textit{utility loss}, and \textit{efficiency reduction}. To this end, federated learning practitioners need tools to measure the three factors and optimize the tradeoff between them to choose the protection mechanism that is most appropriate to the application at hand. Motivated by this requirement, we propose a framework that (1) formulates TFL as a problem of finding a protection mechanism to optimize the tradeoff between privacy leakage, utility loss, and efficiency reduction and (2) formally defines bounded measurements of the three factors. We then propose a meta-learning algorithm to approximate this optimization problem and find optimal protection parameters for representative protection mechanisms, including Randomization, Homomorphic Encryption, Secret Sharing, and Compression. We further design estimation algorithms to quantify these found optimal protection parameters in a practical horizontal federated learning setting and provide a theoretical analysis of the estimation error.

==> 002_Lower_Bound_for_Privacy_Leakage.tex <==
\section{Lower Bound for Privacy Leakage}

\begin{lem}\label{lem: JSBound_app}
Let $P_k^{\calRO}$ and $P^{\calD}_k$ represent the distribution of the parameter of client $k$ before and after being protected. Let $F^{\calA}_k$ and $F^{\calRO}_k$ represent the belief of client $k$ about $S$ after observing the protected and original parameter. Then we have
\begin{align*}
{\text{JS}}(F^{\calA}_k || F^{\calRO}_k)\le \frac{1}{4}(e^{2\xi}-1)^2{\text{TV}}(P_k^{\calRO} || P^{\calD}_k)^2. 
\end{align*}
\end{lem}

\begin{proof}

Let $F^{\calM}_k = \frac{1}{2}(F^{\calA}_k+ F^{\calRO}_k)$. We have

\begin{align*}
{\text{JS}}(F^{\calA}_k || F^{\calRO}_k) & = \frac{1}{2}\left[KL\left(F^{\calA}_k, F^{\calM}_k\right) + KL\left(F^{\calRO}_k,F^{\calM}_k\right)\right]\\
& = \frac{1}{2}\left[\int_{\mathcal{D}_k} f^{\calA}_{D_k}(d)\log\frac{f^{\calA}_{D_k}(d)}{f^{\calM}_{D_k}(d)}ds + \int_{\mathcal{D}_k} f^{\calRO}_{D_k}(d)\log\frac{f^{\calRO}_{D_k}(d)}{f^{\calM}_{D_k}(d)}ds\right]\\
& = \frac{1}{2}\left[\int_{\mathcal{D}_k} f^{\calA}_{D_k}(d)\log\frac{f^{\calA}_{D_k}(d)}{f^{\calM}_{D_k}(d)}ds - \int_{\mathcal{D}_k} f^{\calRO}_{D_k}(d)\log\frac{f^{\calM}_{D_k}(d)}{f^{\calRO}_{D_k}(d)}ds\right]\\
&\le \frac{1}{2}\int_{\mathcal{D}_k}\left|f^{\calA}_{D_k}(d) - f^{\calRO}_{D_k}(d)\right|\left|\log\frac{f^{\calM}_{D_k}(d)}{f^{\calRO}_{D_k}(d)}\right|ds,
\end{align*}
where the inequality is due to $\frac{f^{\calA}_{D_k}(d)}{f^{\calM}_{D_k}(d)}\le \frac{f^{\calM}_{D_k}(d)}{f^{\calRO}_{D_k}(d)}$.





\textbf{Bounding $\left|f^{\calA}_{D_k}(d) - f^{\calRO}_{D_k}(d)\right|$.}

Let $\mathcal U_k = \{w\in\mathcal W_k: dP^{\calD}_k(w) - dP_k^{\calRO}(w)\ge 0\}$, and $\mathcal V_k = \{w\in\mathcal W_k: dP^{\calD}_k(w) - dP_k^{\calRO}(w)< 0\}$.

\red{

For any $w\in\mathcal V_a$, the definition of $\mathcal V_a$ implies that $dP_{\text{fed}}^{\calRO}(w) > dP_{\text{fed}}^{\calD}(w)\ge 0$. Therefore, $w$ belongs to the support of $P_{\text{fed}}^{\calRO}$, which is denoted as $\mathcal W^{\calRO}_{\text{fed}}$. Therefore we have that
\begin{align}\label{eq: subset_relationship_1}
    \mathcal V_a\subset\mathcal W^{\calRO}_{\text{fed}}.
\end{align}

Similarly, we have that
\begin{align}\label{eq: subset_relationship_n}
    \mathcal U_a\subset\mathcal W^{\calD}_a.
\end{align}
}

Then we have 

\begin{align}\label{eq:initial_step_{JS}}
    \left|f^{\calA}_{D_k}(d) - f^{\calRO}_{D_k}(d)\right| &= \left|\int_{\mathcal W_k} g_{D_k|W_k}(d|w, v_a)[d P^{\calD}_k(w) - d P_k^{\calRO}(w)]\right|\nonumber\\
    &= \left|\int_{\mathcal{U}_k} g_{D_k|W_k}(d|w, v_a)[d P^{\calD}_k(w) - d P_k^{\calRO}(w)] + \int_{\mathcal{V}_k} g_{D_k|W_k}(d|w, v_a)[d P^{\calD}_k(w) - d P_k^{\calRO}(w)]\right|\nonumber\\
    %&\le\sup_{w\in\mathcal W^{\calD}_k \setminus \mathcal W^{\calRO}_k} g_{D_k|W_k}(d|w, v_a)\int_{\U} [d P^{\calD}_k(w) - d P_k^{\calRO}(w)] + \inf_{w\in\mathcal W^{\calRO}_k} g_{D_k|W_k}(d|w, v_a)\int_\V[d P^{\calD}_k(w) - d P_k^{\calRO}(w)]\nonumber\\
    &\le\left(\sup_{w\in\mathcal{W}_k} g_{D_k|W_k}(d|w, v_a) - \inf_{w\in\mathcal{W}_k} g_{D_k|W_k}(d|w, v_a)\right)\int_{\mathcal{U}_k} [d P^{\calD}_k(w) - d P_k^{\calRO}(w)].
\end{align}

%\XZ{For HE, $g_{D_k|W_k}(d|w, v_a)\le g_{D_k}(d| v_a)$ for any $w\in\mathcal W$.}

%First, we provide an upper bound for $(\sup_{w} g_{D_k|W_k}(d|w, v_a) - \inf_{w} g_{D_k|W_k}(d|w, v_a))$.%the first term of \pref{eq:initial_step}.
%\textbf{Bounding $\sup_{y} p(d|y) - \inf_{y} p(d|y)$.}

%For any pair of parameters $w\in\mathcal W^{\calD}_k \setminus \mathcal W^{\calRO}_k$ and $w'\in\mathcal W^{\calRO}_k$, we have
Notice that

\begin{align*}
    \sup_{w\in\mathcal W_k} g_{D_k|W_k}(d|w, v_a) - \inf_{w\in\mathcal W_k} g_{D_k|W_k}(d|w, v_a) = \inf_{w\in\mathcal W_k} g_{D_k|W_k}(d|w, v_a)\left|\frac{\sup_{w\in\mathcal W_k} g_{D_k|W_k}(d|w, v_a)}{\inf_{w\in\mathcal W_k} g_{D_k|W_k}(d|w, v_a)}-1\right|.
\end{align*}

%%%%% Using a lemma to illustrate this property
From the definition of $\xi$, we know that for any $w\in\mathcal W_k$,
\begin{align*}
    e^{-\xi}\le\frac{g_{D_k|W_k}(d|w, v_a)}{g_{D_k}(d| v_a)}\le e^{\xi},
\end{align*}

\red{
for any pair of parameters $w\in\mathcal W_k^{\calD}$ and $w'\in\mathcal W_k^{\calRO}$, we have
\begin{align*}
    \frac{g_{D_k|W_k}(d|w, v_a)}{g_{D_k}(d| v_a)} = 1,
\end{align*}

and

\begin{align*}
    e^{-\xi}\le\frac{g_{D_k|W_k}(d|w', v_a)}{g_{D_k}(d| v_a)}\le e^{\xi},
\end{align*}
}




Therefore, for any pair of parameters $w,w'\in\mathcal W_k$, we have
\begin{align*}
    \frac{g_{D_k|W_k}(d|w, v_a)}{g_{D_k|W_k}(d|w', v_a)} = \frac{g_{D_k|W_k}(d|w, v_a)}{g_{D_k}(d| v_a)}/\frac{g_{D_k|W_k}(d|w', v_a)}{g_{D_k}(d| v_a)}\le e^{2\xi}. 
\end{align*}

\red{
Therefore, for any pair of parameters $w\in\mathcal W_k^{\calD}$ and $w'\in\mathcal W_k^{\calRO}$, we have
\begin{align*}
    \frac{g_{D_k|W_k}(d|w, v_a)}{g_{D_k|W_k}(d|w', v_a)} = \frac{g_{D_k|W_k}(d|w, v_a)}{g_{D_k}(d| v_a)}/\frac{g_{D_k|W_k}(d|w', v_a)}{g_{D_k}(d| v_a)}\le e^{\xi}. 
\end{align*}


}




%%%%% Using a lemma to illustrate this property


Therefore, the first term of \pref{eq:initial_step_{JS}} is bounded by

\begin{align}\label{eq: bound_1_term_1_{JS}_ratio}
    \sup_{w\in\mathcal W_k} g_{D_k|W_k}(d|w, v_a) - \inf_{w\in\mathcal W_k} g_{D_k|W_k}(d|w, v_a) \le \inf_{w\in\mathcal W_k} g_{D_k|W_k}(d|w, v_a)(e^{2\xi}-1).
\end{align}

From the definition of total variation distance, we have
\begin{align}\label{eq: bound_1_term_2_{JS}_ratio}
    \int_{\U} [d P^{\calD}_k(w) - d P_k^{\calRO}(w)] = {\text{TV}}(P_k^{\calRO} || P^{\calD}_k).
\end{align}

Combining \pref{eq: bound_1_term_1_{JS}_ratio} and \pref{eq: bound_1_term_2_{JS}_ratio}, we have
\begin{align}\label{eq: bound_for_the_gap}
        |f^{\calA}_{D_k}(d) - f^{\calRO}_{D_k}(d)| &=\left(\sup_{w\in\mathcal W_k} g_{D_k|W_k}(d|w, v_a) - \inf_{w\in\mathcal W_k} g_{D_k|W_k}(d|w, v_a)\right)\int_\U [d P^{\calD}_k(w) - d P_k^{\calRO}(w)]\nonumber\\
        &\le\inf_{w\in\mathcal W_k} g_{D_k|W_k}(d|w, v_a)(e^{2\xi}-1){\text{TV}}(P_k^{\calRO} || P^{\calD}_k).
\end{align}



%\textbf{Bounding the second term of \pref{eq:initial_step}.}



\textbf{Bounding $\left|\log\left(\frac{f^{\calM}_{D_k}(d)}{ f^{\calRO}_{D_k}(d)}\right)\right|.$}

%From \pref{lem: log_upper_bound}, 
We have that

\begin{align}\label{eq: bound_for_log_ratio}
    \left|\log\frac{f^{\calM}_{D_k}(d)}{f^{\calRO}_{D_k}(d)}\right|&\le\frac{|f^{\calM}_{D_k}(d) - f^{\calRO}_{D_k}(d)|}{\min\{f^{\calM}_{D_k}(d), f^{\calRO}_{D_k}(d)\}}\nonumber\\
    &=\frac{|f^{\calA}_{D_k}(d) - f^{\calRO}_{D_k}(d)|}{2\min\{f^{\calM}_{D_k}(d), f^{\calRO}_{D_k}(d)\}}\nonumber\\
    &\le \frac{\inf_{w\in\mathcal W_k} g_{D_k|W_k}(d|w, v_a)(e^{2\xi}-1){\text{TV}}(P_k^{\calRO} || P^{\calD}_k)}{2\min\{f^{\calM}_{D_k}(d), f^{\calRO}_{D_k}(d)\}}\nonumber\\
    &\le \frac{1}{2}(e^{2\xi}-1){\text{TV}}(P_k^{\calRO} || P^{\calD}_k),
\end{align}
where the first inequality is due to \pref{lem: log_upper_bound}, the third inequality is due to $\min\{f^{\calM}_{D_k}(d), f^{\calRO}_{D_k}(d)\}\ge \min\{f^{\calA}_{D_k}(d), f^{\calRO}_{D_k}(d)\}\ge \inf\limits_{\small{w\in\mathcal W_k}} g_{D_k|W_k}(d|w, v_a)$.
%, and $\frac{g_{D_k|W_k}(d|w, v_a)}{g_{D_k}(d| v_a)}\le e^{\xi}$ for any $w\in\mathcal W^{\calRO}_k$.

Combining \pref{eq: bound_for_the_gap} and \pref{eq: bound_for_log_ratio}, we have
\begin{align*}
    {\text{JS}}(F^{\calA}_k || F^{\calRO}_k) & \le  \frac{1}{2}\left[\int_{\mathcal{D}_k} \left|(f^{\calA}_{D_k}(d) - f^{\calRO}_{D_k}(d))\right| \left|\log\frac{f^{\calM}_{D_k}(d)}{f^{\calRO}_{D_k}(d)}\right|ds\right]\\
    &\le \frac{1}{4}(e^{2\xi}-1)^2{\text{TV}}(P_k^{\calRO} || P^{\calD}_k)^2\int \inf_{w\in\mathcal W^{\calRO}_k} g_{D_k|W_k}(d|w, v_a)ds\\
    &\le\frac{1}{4}(e^{2\xi}-1)^2{\text{TV}}(P_k^{\calRO} || P^{\calD}_k)^2.
\end{align*}

\end{proof}


\begin{lem}
\begin{align*}
    \sqrt{{\text{JS}}(F^{\calRO}_k || F^{\calO}_k)}\le\epsilon_p + \frac{1}{2}(e^{2\xi}-1){\text{TV}}(P_k^{\calRO} || P^{\calD}_k).
\end{align*}
The larger $n$ is, the smaller the privacy leakage is. 
\end{lem}
\begin{proof}
Recall the triangle inequality shows that 
\begin{align*}
    \sqrt{{\text{JS}}(F^{\calRO}_k || F^{\calO}_k)} - \sqrt{{\text{JS}}(F^{\calA}_k || F^{\calO}_k)}\le \sqrt{{\text{JS}}(F^{\calA}_k || F^{\calRO}_k)},
\end{align*}

where $\sqrt{{\text{JS}}(F^{\calRO}_k || F^{\calO}_k)}$ is a problem-dependent constant, $\sqrt{{\text{JS}}(F^{\calA}_k || F^{\calO}_k)}$ represents the privacy leakage, and $\sqrt{{\text{JS}}(F^{\calA}_k || F^{\calRO}_k)}\le \frac{1}{2}(e^{2\xi}-1){\text{TV}}(P_k^{\calRO} || P^{\calD}_k)$. Therefore, we have that
\begin{align*}
    \sqrt{{\text{JS}}(F^{\calRO}_k || F^{\calO}_k)}&\le\epsilon_p + \frac{1}{2}(e^{2\xi}-1){\text{TV}}(P_k^{\calRO} || P^{\calD}_k).
\end{align*}

% For the encryption scheme, given any parameter $w$, the information gain of the attacker is close to zero due to semantic security. In fact, the information gain of the attacker is related to the guessing range of the attacker. It implies that the privacy leakage decreases with $n$.
\end{proof}

==> estimation_for_c2_prepare_version.tex <==
\red{
\begin{lem}[The Estimation Error of $C_2$]
  We have that
  \begin{align}
      |\hat C_2 - C_2|\le 3\epsilon C_2,
  \end{align}
  where $\epsilon = $.
\end{lem}
\begin{proof}

\begin{align}
    \xi_k & = \max_{d \in \mathcal{D}_k} \left|\log\left(\frac{f_{D_k|W_k}(d|w^*)}{f_{D_k}(d)}\right)\right|.
\end{align}

We approximate $\xi_k$ by:
\begin{align}
    \hat\xi_k & = \max_{d \in \mathcal{D}_k} \left|\log\left(\frac{\hat f_{D_k|W_k}(d|w^*)}{f_{D_k}(d)}\right)\right|.
\end{align}

\red{
Recall that 
\begin{align}
    \hat f_{D_k|W_k}(d|w^*) = 
\end{align}
}

First, we show that
\begin{align}
    |f_{D_k|W_k}(d|w^*) - \hat f_{D_k|W_k}(d|w^*)|\le\gamma f_{D_k|W_k}(d|w^*). 
\end{align}

Therefore, we have that
\begin{align}
    |\hat\xi_k - \xi_k|\le\epsilon, 
\end{align}
where $\epsilon = $.

$\hat\kappa_3=\max_{k\in [K]}\hat\xi_k$. Therefore,
\begin{align}
    |\hat\kappa_3 - \kappa_3|\le\epsilon. 
\end{align}

We compute $C_2$ by
\begin{align}
    \hat C_2 = \frac{1}{2}(e^{2\hat\kappa_3}-1).
\end{align}
Therefore, we have that
\begin{align*}
    |\hat C_2 - C_2| & \le |\frac{1}{2}(e^{2\kappa_3 + \epsilon}-1) - \frac{1}{2}(e^{2\kappa_3}-1)|\\
    & = \frac{1}{2} e^{2\kappa_3} |e^{\epsilon} - 1|\\
    &\le\frac{\epsilon}{2} e^{2\kappa_3}.
\end{align*}
From
\begin{align}
    \frac{e^{2\kappa_3}}{6}\le \frac{e^{2\kappa_3}}{2} - 1, 
\end{align}
we further have
\begin{align}
    |\hat C_2 - C_2|\le 3\epsilon C_2. 
\end{align}
\end{proof}
}

==> sections/01-introduction.tex <==
\section{Introduction}
\label{sec:introduction}


{Modern machine learning techniques are data-hungry, and it is not uncommon to use trillion bytes of data in developing large pre-trained machine learning models, e.g., for natural language processing \cite{devlin2018bert,dong2019unified} or image processing \cite{karras2019style,chen2021pre}. For a large variety of machine learning applications, for instance, in social media or finance use cases, data are often distributed across multiple devices or institutions.} Collecting such data onto a central server for training will incur additional communication overhead, management and business compliance costs, privacy issues, and even regulatory and judicial issues such as General Data Protection Regulation (GDPR)\footnote{GDPR is applicable as of May 25th, 2018 in all European member states to harmonize data privacy laws across Europe. https://gdpr.eu/}. Federated Learning (FL) has been introduced as an effective technology to allow multiple parties to jointly train a model \textit{without gathering or exchanging private training data among different parties}. Moreover, it is also required that information exchanged during the learning or inference stages \textit{do not disclose private data owned by respective parties to semi-honest adversaries} (for a formal definition, see Sect. \ref{sec:related:attack}), who aim to espy or infer other parties' private data from exchanged information. The requirements as such constitute the primary mandate for a novel statistical framework of privacy-preserving federated learning as illustrated in this article. 

From an information theory point of view, the amount of information about private data that a semi-honest party can infer from exchanged information is inherently determined by the \textit{statistical dependency} between private data and publicly exchanged information. %\HL {see \pref{prop: tradeoff-extremecase}}.
Recent studies have shown that semi-honest adversaries can exploit this dependency to recover the private training images with pixel-level accuracy from exchanged gradients of learned models, e.g., by using Bayesian inference attacks (see Sect. \ref{sec:Bayesian inference attack} and \cite{zhu2019dlg,zhu2020deep,he2019model} for details). 
Taking such threat models into account, we therefore reiterate that a 
\textit{secure federated learning} (SFL) scheme must a) support multiple parties to jointly train models and to make joint inferences \textit{without exchanging private data}; b) have \textit{clearly defined threat models and security guarantees} under these models.
%; c) include mechanisms for \textit{auditing and managing the models} thus generated\footnote{The topic of auditing and managing the models itself is out of the scope of the present article though and we will report our research along this direction elsewhere.}.



In this article, we consider a \textit{horizontal federated learning} \cite{yang2019federated}, or a \textit{cross-device federated learning} \cite{DBLP:journals/ftml/KairouzMABBBBCC21} setting, in which multiple \textit{clients} upload respective local models or model updates to an \textit{aggregator}\footnote{We assume the existence of a centralized aggregator for the brevity of analysis. Yet the analysis is also applicable to the decentralized federated learning setting in which model aggregation is performed without an aggregator. Detailed discussion on this setting is out of the scope of this article though and will be reported elsewhere.}, who is responsible for %provides computing or service (e.g., server offers 
aggregating multiple local models into a global model. There are a variety of application scenarios that use this scheme for federated learning \cite{mcmahan2016federated, mcmahan2017communication, yang2019federated_new}.
%In particular, we consider the model learning process which iterates between the local model update and global aggregation sub-processes, in a privacy-preserving manner, until the global model converges.
The fundamental privacy-preserving requirement is to maintain potential \textit{privacy loss} below an acceptable level. This is achieved by reducing the dependency between the exchanged model information and private data. The reduced dependency, however, makes the aggregated global model less accurate and leads to \textit{utility loss}, such as a loss in model accuracy, as compared to a global model trained without using any protection. Severely degraded model utility indeed defeats the purpose of federated learning in the first place. We therefore propose in this article a unified statistical framework to analyze the privacy-utility trade-off on a rigorous theoretical foundation. The main results of our research are summarized as follows (also see Fig. \ref{fig:framework} for a pictorial summary):

\begin{itemize}
\item First, we formulate the privacy leakage attack \cite{zhu2019dlg,zhu2020deep,he2019model} through a \textbf{Bayesian inference attack} perspective (Def. \ref{def:attackA}) \cite{geman1984stochastic,wasserman2004bayesian}. A privacy metric called \textbf{Bayesian Privacy} is then proposed to quantify the additional amount of information about private data that a semi-honest adversary might gain by observing publicly exchanged information. Specifically, the information gain for adversaries i.e., \textbf{Bayesian privacy leakage} (Def. \ref{defi: average_privacy_JSD}) is measured by distances between distributions of adversaries' \textit{prior} and \textit{posterior} beliefs about private data. 
Also, an upper bound of Bayesian privacy leakage called \textbf{$\epsilon$-Bayesian Privacy} provides the privacy-preserving guarantee regardless of any Bayesian inference attack that may be launched by semi-honest adversaries. 
%Both \textit{threat models} for adversaries and \textit{security models} against adversaries are taken into account in the proposed Bayesian privacy formulation. 
%lay down the foundation for rigorous analysis illustrated in this article. 
%Instead of using the asymmetric Kullback–Leibler divergence, we make use of symmetrical metrics including $l1$ distance, Jensen-Shannon (JS) divergence\footnote{The square root of Jensen-Shannon divergence (aka Jensen-Shannon Distance) is a metric satisfying the triangular inequality which is used to prove main results in Sect. \ref{sec:framework}} and generalized JS divergence (see Sect. \ref{sect:privacy leakage}).
%Technically, the abstract Bayesian Privacy framework allows such distances to be measured by a variety of metrics including $l1$ distance, Jensen-Shannon (JS) divergence, or generalized JS divergence (see Sect. \ref{sect:tradeoff} for details);  
%under the Bayesian inference attack in terms of capturing the privacy threat by a user who releases some information. Specifically, 
%Bayesian Privacy measures the distance between prior and posterior beliefs of attackers after observing exposure information.

\item Second, we put forth a statistical framework to cast the optimal privacy-utility trade-off as a constrained optimization problem
in which a \textit{utility loss} (Def. \ref{defi: utility_loss}) is minimized subject to a preset upper bound of Bayesian privacy leakage (i.e. \textbf{$\epsilon$-Bayesian Privacy}) constraint (see Sect. \ref{sec: optimzation problem}). A theoretical analysis of the trade-off is then manifested as \textbf{Theorem \ref{thm: utility-privacy trade-off_JSD_mt}}, which dictates that a) a weighted sum of the privacy loss and utility loss is greater than a problem-dependent non-zero constant; b) relative weights between the privacy loss and utility loss depend on multiple factors including Bayesian inference attacks adversaries may launch, %\XZ{encounter?}, 
protection mechanisms adopted as well as distributions of the training and testing data. %\XZ{do we consider test data}. 
That is to say, in principle,\textit{ one has to trade a decrease of the privacy-loss with a certain degree of increase of the utility loss, and vice versa}\footnote{This principle bears an intriguing similarity to the no free lunch theorem for optimization and machine learning \cite{wolpert1997no}, which inspire us to name Theorem \ref{thm: utility-privacy trade-off_JSD_mt} “No free lunch theorem (NFL) for security and utility” in federated learning.}. 
%provided by \pref{thm: utility-privacy trade-off_JSD_mt}.
%where the utility loss is minimized given \textit{Bayesian privacy} constraint. 

%Specifically, inspired by the definition of Semantic Security \cite{goldwasser1984probabilistic}, our framework measures the distance between prior and posterior belief of attackers after observing exposure information. Moreover, the privacy threat our framework considers not only query but also active attacking\XZ{considers not only query but also active attacking, this sentence, how to modify?}, i.e. Bayesian inference attack. Additionally, our framework could cover different protection mechanisms including randomization, sampling, and Encryption. 
\item Third, the general principle of Theorem \ref{thm: utility-privacy trade-off_JSD_mt} is applied to give quantitative analysis of the trade-off under specific privacy-protection mechanisms, including \textit{Randomization} \cite{geyer2017differentially,truex2020ldp,abadi2016deep}, \textit{Sparsity} \cite{shokri2015privacy, gupta2018distributed, thapa2020splitfed} and \textit{Homomorphic Encryption (HE)} \cite{gentry2009fully,batchCryp} (see \textbf{Theorem \ref{thm: privacy-utility-tradeoff-random}, \ref{thm: privacy-utility-tradeoff-sparsity} and \ref{thm:tradeoff-HE}}). These theoretically justified results are of interest in their own rights. On the other hand, they are of pragmatic values in serving as practical guidance to the design of federated learning algorithms under various scenarios (see Sect. \ref{sec:application} for applications). 
%\HL{to confirm?: We refer readers to Appendix \ref{?} in which a couple of applications are briefly outlined. }
%It turns out that different protection mechanisms lead to quantitatively different trade-offs are illustrated, respectively, by Theorem \ref{thm: privacy-utility-tradeoff-random}, \ref{thm: privacy-utility-tradeoff-sparsity} and \ref{thm:tradeoff-HE}.  %\LF{Moreover, ...?}


%Among three protection mechanisms, HE provides the most favorable privacy-utility trade-off in terms of  
%Quantitative analysis of the trade-off between utility loss and Bayesian Privacy for different protection mechanisms is offered in this paper.
\end{itemize}

To our best knowledge, the proposed Bayesian Privacy formulation is the first unified framework that explicitly considers both \textit{threat models} (attacking mechanisms) and \textit{security models} (protection mechanisms). It is also the first that is applicable to different privacy-protection mechanisms including randomization \cite{geyer2017differentially,truex2020ldp,abadi2016deep}, Sparsity \cite{shokri2015privacy, gupta2018distributed, thapa2020splitfed} and Homomorphic Encryption \cite{gentry2009fully,batchCryp}. {The rest of the article is organized as follows: Sect. \ref{sec:related} reviews existing works related to privacy measurements and federated learning; Sect. \ref{sec:framework} illustrates the statistical framework based on Bayesian inference attacks and protection mechanisms; %Following the Bayesian Privacy framework, 
Sect. \ref{sect:tradeoff} illustrates the quantification of the privacy-utility trade-off (Theorem \ref{thm: utility-privacy trade-off_JSD_mt}), the applications of the trade-off on different protection mechanisms are further presented in Sect. \ref{sec:application}; The comparison of Bayesian Privacy with other privacy measurements is presented in Sect. \ref{sect:compare-BP}. Finally, Sect. \ref{sec:conclusion} concludes the article with discussions on future research plans.}

\begin{figure}[h]
\centering
\includegraphics[width = 0.9\columnwidth]{figures/framework.pdf}
\caption{Outline of the proposed SFL framework based on Bayesian inference attack and the privacy-utility trade-off.} \label{fig:framework}
\end{figure}



==> sections/04-framework.tex <==
\section{A general framework for the Privacy-Utility Trade-Off}\label{sect:tradeoff}
In Sect. \ref{sec:framework}, we have introduced the definition of privacy leakage and utility loss in SFL. In this section, we first lay down the rigorous analysis of the trade-off between Bayesian privacy leakage and utility loss (no free lunch theorem). Then we formulate the \textit{privacy-utility trade-off} as an optimization problem, which minimizes the utility loss under the $\epsilon$-Bayesian privacy constraint. Finally, we apply the proposed no free lunch theorem between Bayesian privacy leakage and utility loss into three protection mechanisms in SFL.


\subsection{Theoretical Analysis for Privacy-Utility Trade-Off}\label{subsect:PU-tradeoff}

The idea of privacy-preserving is to modify the unprotected information and guarantee that the private data cannot be disclosed to semi-honest adversaries. In order to protect privacy, the protected information denoted as $W^{\calD}_k$ is shared. %sampled from distribution $P^{\calD}_k$ 
The utility loss quantifies the increase of expected average loss incurred by the released information $W^{\calD}_k$ compared with the utility caused by $W^{\calRO}_k$. 
Note that $W^{\calD}_k$ and $W^{\calRO}_k$ respectively follow distributions $P^{\calD}_k$ and $P_k^{\calRO}$. In this setting, we want to characterize the limitation of privacy-preserving mechanisms. It requires to measure the amount of utility that is inevitable to lose in order to protect privacy. Intuitively, the larger the change exerted on $W^{\calRO}_k$ is, the more secure the privacy protection is, and meanwhile, the less accurate the output is. We first measure the extent of modification using the total variation distance between the unprotected distribution and the protected distribution. Then, we use this distance as a key element for connecting the privacy leakage and the utility loss.
Note that the union of $\mathcal W_k^{\calD}$ (the support of $P_k^{\calD}$) and $\mathcal W_k^{\calRO}$ (the support of $P_k^{\calRO}$) is denoted as $\calW_k$.


% \begin{assumption}
% Assume that the utility of the aggregated parameter achieves the maximal value at the convergence step.
% \end{assumption}


% \begin{definition}[Optimal parameters]
% Let $\mathcal W^{*}_a$ represent the set of parameters achieving the maximum utility. Specifically, 
% \begin{align*}
%     \mathcal W^{*}_a = \{w\in\mathcal W_a: U_a(w) = U_a^{*}\},
% \end{align*}
% where $U_a(w) = \mathbb E_{S_a}\frac{1}{|S_a|}\sum_{s\in S_a}U(w,s)$ is the expected utility taken over $S_a$ sampled from distribution $P_a$, and $U_a^{*} = \max_{w\in\mathcal W_a} U_a(w)$ represents the maximum utility over $\mathcal W_a$.
% \end{definition}



\begin{definition}[Optimal parameters]
Let $\mathcal W^{*}_a$ represent the set of parameters achieving the maximum utility. Specifically, 
\begin{align*}
    \mathcal W^{*}_a = \argmax_{w\in\mathcal W_a}\frac{1}{K}\sum_{k=1}^K U_k(w),
\end{align*}
where $U_k(w) = \mathbb{E}_{S_k}\frac{1}{|S_k|}\sum_{s\in S_k}U(w,s)$ is the expected utility taken over $S_k$ sampled from distribution $P_k$.
\end{definition}



%\XZ{
% \begin{definition}[Optimal parameters]
% Let $\mathcal W^{*}_a$ represent the set of parameters achieving the maximum utility. Specifically, 
% \begin{align*}
%     \mathcal W^{*}_a = \{w\in\mathcal W_a: \frac{1}{K}\sum_{k=1}^K U_k(w) = U^{*}\},
% \end{align*}
% where $U_k(w) = \mathbb E_{S_k}\frac{1}{|S_k|}\sum_{s\in S_k}U(w,s)$ is the expected utility taken over $S_k$ sampled from distribution $P_k$, and $U^{*} = \max_{w\in\mathcal W_a}\frac{1}{K}\sum_{k=1}^K U_k(w)$ represent the maximum utility over $\mathcal W_a$.
% %all unprotected parameters and protected parameters. 
% % let
% % Assume that the utility resulting from any parameter in $\mathcal W^{\calRO}_k$ achieves the maximal value. Specifically,
% \end{definition}






% \begin{assumption}
% Assume that the utility resulting from any parameter in $\mathcal W^{\calRO}_k$ achieves the maximal value. Specifically, for any $w\in\mathcal W^{\calRO}_k$, it holds that

% \begin{align*}
% U_k(w) = \max_{w'\in\mathcal W_k} U_k(w').
% \end{align*}

% \end{assumption}

\begin{definition}[Near-optimal parameters]\label{defi: neighbor_set}
Let $\calW^{\calD}_a$ represent the support of the protected distribution of the aggregated model information. Given a non-negative constant $c$, the \textit{near-optimal parameters} is defined as
$$\calW_{c} = \left\{w\in\calW^{\calD}_a: \left|\frac{1}{K}\sum_{k=1}^K  U_k(w^{*})-\frac{1}{K}\sum_{k=1}^K U_k(w)\right|\le c, \forall w^{*}\in\mathcal W^{*}_a\right\}.$$

% $\calW_{c} = \{w\in\calW^{\calD}_k: 0<| U_k(w^{*})-U_k(w)|\le c, \forall w^{*}\in\mathcal W^{*}_k\}$.






% , and $\Delta_k$ is a maximum positive constant satisfying that
% \begin{align}
% \int_{\calW_k^{\calD}} p^{\calD}_{W_k}(w)\one\{w\in \calW^{\calD}_k\} dw\le\frac{{\text{TV}}(P_a^{\calRO} || P_a^{\calD} )}{2}.
% \end{align}
\end{definition}

\begin{assumption}\label{assump: assump_of_Delta}
%Assume 
Let $\Delta$ be the \textit{maximum} constant that satisfies
% \begin{align}
% \int_{\calW_k^{\calD}} p^{\calD}_{W_k}(w)\one\{w\in\calW_{\Delta_k}\} dw\le\frac{{\text{TV}}(P_a^{\calRO} || P_a^{\calD} )}{2},
% \end{align}

% \begin{align}
%      \int_{\mathcal W^{\calD}_a} p^{\calD}_{W_a}(w)\one\{w\in\calW_{\Delta_k}\} dw\le\frac{{\text{TV}}(P_a^{\calRO} || P_a^{\calD} )}{2},
% \end{align}

\begin{align}
     \int_{\mathcal W^{\calD}_a} p^{\calD}_{W_a}(w)\one\{w\in\calW_{\Delta}\} dw\le\frac{{\text{TV}}(P_a^{\calRO} || P_a^{\calD} )}{2},
\end{align}


where $p^{\calD}_{W_a}$ represents the probability density function of the protected model information $W_a^\calD$. We assume that $\Delta$ is positive, i.e., $\Delta >0$.
%Assume that the bounded neighboring utility parameter set exists for each client.
% Assume that the neighborhood set $\calW_{\Delta_k}$ as defined in \pref{defi: neighbor_set} is a sub-optimal parameter set. That is, $\Delta_k$ is a positive constant for each client $k$.
\end{assumption}
\textbf{Remark:}\\
(1) This assumption implies that the cumulative density of the near-optimal parameters as defined in Def. \ref{defi: neighbor_set} is bounded. This assumption excludes the cases where the utility function is constant or indistinguishable between the optimal parameters and a certain fraction of parameters.  \\
(2) Note that $\Delta_k$ is independent of the threat model of the adversary and $\Delta_k$ is a constant when the protection mechanism, the utility function, and the data sets are fixed.\\



% \textbf{Remark:} This assumption implies that the cumulative density of the neighboring utility parameters as defined in Def. \ref{defi: neighbor_set} is bounded. In other words, we assume that majority of model parameters are sub-optimal in terms of utilities obtained with these parameters. This assumption excludes the cases where the utility function is constant or indistinguishable between the optimal parameters $W_k^*$ and the majority of model parameters.  \\
% \textbf{Remark:} Note that $\Delta_k$ is independent of the threat model of the adversary.










% \begin{definition}[Bounded neighboring utility parameters]\label{defi: neighbor_set}
% The \textit{Bounded neighboring utility parameters} is defined as $\calW_{\Delta_k} = \{w\in\calW^{\calD}_k: 0<| U_k(w^{*})-U_k(w)|\le\Delta_k, \forall w^{*}\in\mathcal W^{*}_k\}$, and $\Delta_k$ is a maximum positive constant satisfying that
% \begin{align}
% \int_{\calW_k^{\calD}} p^{\calD}_{W_k}(w)\one\{w\in \calW^{\calD}_k\} dw\le\frac{{\text{TV}}(P_a^{\calRO} || P_a^{\calD} )}{2}.
% \end{align}
% \end{definition}
% \textbf{Remark:} This definition implies that the cumulative density of the parameters with utility $\Delta_k$ smaller than that of the optimal utility parameters is bounded.\\
% \textbf{Remark:} Note that $\Delta_k$ is independent of the threat model of the adversary.

% \begin{assumption}\label{assump: assump_of_Delta}
% Assume that the bounded neighboring utility parameter set exists for each client.
% % Assume that the neighborhood set $\calW_{\Delta_k}$ as defined in \pref{defi: neighbor_set} is a sub-optimal parameter set. That is, $\Delta_k$ is a positive constant for each client $k$.
% \end{assumption}





%depends on the protection mechanism $\mathcal M_k$, the utility $U_k$, and the data set $\mathcal D_k$.

%}

% For each client $k$, we use $\Delta_k$ to measure the discrepancy between the utility of most parameters (weighted using the probability density) and the maximal utility. In other words, the utility of most parameters is $\Delta_k$ smaller than that of the optimal parameters that client $k$ protects.

% \begin{assumption}[Positive Majority Discrepancy]\label{assump: assump_of_Delta}
% For each client $k$, let $\Delta_k>0$ be the positive maximum constant satisfying that
% \begin{align}
% \int_{\calW_{\Delta_k}} p^{\calD}_{W_k}(w) dw\le\frac{{\text{TV}}(P_a^{\calRO} || P_a^{\calD} )}{3},
% \end{align}
% where $\calW_{\Delta_k} = \{w\in\calW^{\calD}_k: U_k(w^{\calRO})-U_k(w) \in[0, \Delta_k],\forall w^{\calRO}\in\mathcal W^{\calRO}_k\} \cup \{w\in\calW^{\calD}_k: U_k(w)> U_k(w^{\calRO}),\exists w^{\calRO}\in\mathcal W^{\calRO}_k\}$. 
% %We assume that $\Delta_k>0$ for each client $k$.
% \end{assumption}




%We recall that $P_k^{\calRO}$ and $P^{\calD}_k$ represent the distributions of the model information of client $k$ before and after being protected, $P_a^{\calRO}$ and $P_a^{\calD}$ represent the distribution of the aggregated model information of client $k$ before and after being protected, $F^{\calB}_k$ represent the prior belief of client $k$ about $S$ and $F^{\calRO}_k$ represent the belief of client $k$ about $S_k$ after observing the exposed information without any protection. The following theorem illustrates that the summation of the average privacy leakage of the clients and the utility loss is lower bounded by a problem-dependent constant.\\ 

The following theorem represents the central result of this work. As a form of the \textit{No Free Lunch (NFL)} theorem, it states that privacy-protection and utility enhancement of a joint model in our semi-honest SFL setting is bounded by a constant. If one increases privacy protection, one risks losing some utility of the joint model, and vice versa. 

\begin{thm}[No free lunch theorem (NFL) for security and utility]\label{thm: utility-privacy trade-off_JSD_mt} Let $\epsilon_p$ be defined in Def. \ref{defi: average_privacy_JSD}, we have that
\begin{align}\label{eq: total_variation-privacy trade-off}
C_1\le\epsilon_{p} + \frac{1}{K}\sum_{k=1}^K \frac{1}{2}(e^{2\xi}-1)\cdot {\text{TV}}(P_k^{\calRO} || P^{\calD}_k).
\end{align}

Furthermore, let $\epsilon_u$ be defined in Def. \ref{defi: utility_loss} at the convergence step, with \pref{assump: assump_of_Delta} we have that
%Furthermore, assuming that $\mathcal V_k\subset \mathcal W^{\calRO}_k$ for each client $k$, where $\mathcal V_k = \{w\in\mathcal W_k: dP^{\calD}(w) - dP^{\calRO}(w)\le 0\}$. We have that
\begin{align}\label{eq: total_variation-privacy trade-off_mt}
 C_1 \le\epsilon_{p} + C_2\cdot \epsilon_{u},
\end{align}
in which
\begin{itemize}
%\item $\epsilon_{p} = \frac{1}{K}\sum_{k=1}^K \epsilon_{p,k}$ represents the average privacy leakage over all clients;
%\item $\epsilon_u$ represents the utility loss given in \pref{defi: utility_loss};
\item $\xi = \max_{k\in [K]} \xi_k$, where $\xi_k = \max_{w\in \mathcal{W}_k, s \in \mathcal{S}_k} \left|\log\left(\frac{f_{S_k|W_k}(s|w)}{f_{S_k}(s)}\right)\right|$ represents the maximum privacy leakage over all possible information $w$ released by client $k$, and $[K] = \{1,2,\cdots, K\}$. $\xi$ is a constant independent of the protection and attack mechanisms;

\item $C_1 = \frac{1}{K}\sum_{k=1}^K \sqrt{{\text{JS}}(F^{\calRO}_k || F^{\calO}_k)}$ is a constant 
%for a given problem independent of protection mechanism, which represents 
representing the averaged square root of JS divergence between the distribution of the unprotected parameter of client $k$ and the prior distribution of the adversary's belief about the private information. This constant is independent of the protection mechanisms. %for a given problem.  
% are fixed;

\item $C_2 = \frac{\gamma}{4\Delta}(e^{2\xi}-1)$ is a constant once the protection mechanisms, the utility function, and the data sets are fixed, where $\gamma = \frac{\sum_{k=1}^K {\text{TV}}(P_k^{\calRO} || P^{\calD}_k)}{{\text{TV}}(P^{\calRO}_a || P^{\calD}_a )}$\footnote{see details of analyzing of the value of $\gamma$ in Appendix \ref{sec:proof-random-app}}. 
%Note that $\Delta$ is a constant independent of the attacking ability of the adversary.
\end{itemize}
\end{thm}

\pref{thm: utility-privacy trade-off_JSD_mt} illustrates that the summation of the average privacy leakage of the clients and the utility loss is lower bounded by a problem-dependent constant. As shown in Fig. \ref{fig: flowchart}, Eq. \eqref{eq: total_variation-privacy trade-off_mt} is based on the triangle inequality of the Jensen-Shannon measure adopted in Bayesian privacy leakage \ref{thm: utility-privacy trade-off_JSD_mt}. It essentially dedicates that \textit{one has to trade a decrease of the privacy leakage ($\epsilon_{p}$) with a certain degree of the increase of the utility loss ($\epsilon_u$) and vice versa}. This principle bears an intriguing similarity to the no free lunch %\XZ{Maybe No free lunch should be modified as "no free lunch"} 
theorem for optimization and machine learning \cite{wolpert1997no}, which dedicated that ``if an algorithm performs well on a certain class of problems then it necessarily pays for that with degraded performance on the set of all remaining problems''. We therefore name Eq. \eqref{eq: total_variation-privacy trade-off_mt} ``no free lunch theorem (NFL) for security and utility'' in federated learning. 


\textbf{Remark:} ${\text{TV}}(P_k^{\calRO} || P^{\calD}_k)$ in Eq. \eqref{eq: total_variation-privacy trade-off} provides an upper bound of the modification brought by the protection mechanism, in terms of the distance between distributions of model information with and without protection methods being applied.
% (2) This loss is measured only when the global model converges i.e. with no more improvements in the measured utility.\\
% (2) As shown in Fig. \ref{fig: flowchart} the Eq. \eqref{eq: total_variation-privacy trade-off_mt} is based on the triangle inequality of the Jensen-Shannon measure adopted in Bayesian privacy leakage \ref{thm: utility-privacy trade-off_JSD_mt}. It essentially dedicates that \textit{one has to trade a decrease of the privacy leakage ($\epsilon_{p}$) with a certain degree of the increase of the utility loss ($\epsilon_u$) and vice versa}. This principle bears an intriguing similarity to the no free lunch %\XZ{Maybe No free lunch should be modified as "no free lunch"} 
% theorem for optimization and machine learning \cite{wolpert1997no}, which dedicated that ``if an algorithm performs well on a certain class of problems then it necessarily pays for that with degraded performance on the set of all remaining problems''. We therefore name Eq. \eqref{eq: total_variation-privacy trade-off_mt} ``No free lunch theorem (NFL) for security and utility'' in federated learning. 

%The following figure illustrates the relationship between the utility loss and the privacy leakage.

\begin{figure}[t]
\centering
\includegraphics[width = 0.8\columnwidth]{figures/proof.pdf}
\vspace{-5mm}
\caption{$\epsilon_{p, k} = \sqrt{{\text{JS}}(F^{\calA}_k || F^{\calO}_k)}$ as is introduced in Def. \ref{defi: average_privacy_JSD}. Notice that the square root of the Jensen-Shannon divergence satisfies the triangle inequality. It implies that the summation of $\epsilon_{p,k}$ and $\sqrt{{\text{JS}}(F^{\calA}_k || F^{\calRO}_k)}$ is at least $\sqrt{{\text{JS}}(F^{\calRO}_k || F^{\calO}_k)}$, which is a problem-dependent constant. Moreover, $\sqrt{{\text{JS}}(F^{\calA}_k || F^{\calRO}_k)}$ is at most $\frac{1}{2}(e^{2\xi}-1)\cdot\text{TV}(P_k^{\calRO} || P^{\calD}_k)$. Consequently, the summation of $\epsilon_{p,k}$ and $\frac{1}{2}(e^{2\xi}-1)\cdot\text{TV}(P_k^{\calRO} || P^{\calD}_k)$ is at least $\sqrt{{\text{JS}}(F^{\calRO}_k || F^{\calO}_k)}$. The total variation distance between the unprotected distribution and protected distribution is then used as a key element for connecting the privacy leakage and the utility loss.}
\label{fig: flowchart}
\end{figure}


% {eq: total_variation-privacy trade-off_mt}

\subsection{Privacy-Preserving Optimization} \label{sec: optimzation problem}
In the privacy-preserving machine learning scenario, clients aim to maintain maximal possible model utility without disclosing private information beyond an acceptable level. 
%protect the parameters that guarantee a certain amount of utility and leakages an intolerable amount of private information simultaneously. 
We can view this trade-off as an optimization problem. The goal is to minimize the utility loss subject to the privacy-preserving constraint. Let the Bayesian privacy leakage $\epsilon_{p}$ be defined as Def. \ref{defi: average_privacy_JSD}, %{def:relaxed SS}
we say a SFL system guarantees $\mathbf{\epsilon}$-\textbf{Bayesian Privacy} if it holds that 
\begin{equation}\label{eq:ep-bayes-privacy}
\epsilon_{p} \leq \epsilon.
\end{equation}
%}
${\epsilon}$-{Bayesian Privacy} guarantees that the Bayesian privacy leakage of client $k$ never exceeds a prescribed threshold $\epsilon$ as the security requirement. For a federated machine learning system, the goal is to find a protection mechanism $M$ that achieves the minimum aggregated utility loss. These two requirements can be cast as a constrained optimization problem over the protection mechanism:% $\calM$:
%\paragraph{Guarantee the existence of trade-off} Given privacy level $\xi$, the optimization problem for client $k$ could be formulated as finding a distribution $P^{\calD}_k$ achieving the minimum loss of utility,

%Given the maximum privacy leakage, we aim at minimizing the utility loss. The optimization problem could be written as:
\begin{align} \label{eq: key_constraint_upper_bound}
\begin{array}{r@{\quad}l@{}l@{\quad}l}
\quad\min\limits_{M}&\epsilon_{u}: = \frac{1}{K}\sum_{k=1}^K [U_k(P_a^{\calRO}) - U_k(P_a^{\calD})],\\
\text{s.t.} & \epsilon_p = \frac{1}{K}\sum_{k = 1}^K \sqrt{{\text{JS}}(F^{\calA}_k || F^{\calO}_k)}\le\epsilon.\\
%&C_1 - \frac{1}{K}\sum_{k=1}^K \frac{1}{2}(e^{2\xi}-1)\cdot {\text{TV}}(P_k^{\calRO} || P^{\calD}_k) < \epsilon
%, \quad\forall k\in [1,2,\cdots,K]
%&\int_{\mathcal W_k}f_{W_k|S_k}(w|s) = 1, \quad\forall s\in \mathcal S_k,\\
%&f_{W_k|S_k}(w|s)\ge 0, \quad\forall w\in \mathcal W_k, \forall s\in \mathcal S_k,\\
\end{array}
\end{align}

\textbf{Remark:}

(1) The constant $\epsilon$ imposed in Eq. \eqref{eq: key_constraint_upper_bound} provides a privacy security guarantee that one can achieve, regardless of a variety of Bayesian inference attacks that may be launched by adversaries. 

(2) This constrained optimization problem is closely related to the optimization formulated \cite{du2012privacy} which instead aims to minimize the information leakage while the utility loss is guaranteed to be less than a given threshold.


\iffalse
\begin{lem}\label{lem: d{\text{TV}}_bound_maintext}

Let $f^{\calA}_{S_k}(s) = \int_{\mathcal{W}} f_{S_k|W_k}(s|w)dp^{\calP}_{W_k}(w)$, and $f^{\calRO}_{S_k}(s) = \int_{\mathcal{W}} f_{S_k|W_k}(s|w)dP^{\calRO}_{W_k}(w)$, where $S$ represents the private information, and $W$ represents the information. For any $\xi\ge 0$, let $f_{W|S}(\cdot|\cdot)$ be a privacy preserving mapping that guarantees $\xi$-maximum Bayesian privacy. That is,
\begin{align*}
|f_{S_k|W_k}(s|w) - f_{S_k}(s)|\le \xi,
\end{align*}
for any $w\in\mathcal W$ and any $s\in\mathcal S$. 
Then, we have
\begin{align*}
||F^{\calA}_k - F^{\calRO}_k||_{\text{{\text{TV}}}} \le \xi\cdot e^{\xi}||P_k^{\calRO} - P^{\calD}_k||_{\text{{\text{TV}}}}.
\end{align*}
\end{lem}
\fi


\iffalse
\textbf{Remark:} When $P^{\calD}_k = P_k^{\calRO}$, the privacy leakage $\epsilon_{p,k} = \sqrt{{\text{JS}}(F^{\calA}_k || F^{\calO}_k)} = \sqrt{{\text{JS}}(F^{\calRO}_k || F^{\calO}_k)}$ achieves the largest value $1$ No! We should use the other definition.


\begin{defi}[Average privacy leakage]\label{defi: distance_posterior_prior_true}
The average privacy leakage is defined as
\begin{align}\label{eq: distance_posterior_prior_true}
\epsilon_{p,k} = \sqrt{{\text{JS}}(F^{\calO}_k, F^{\calRO}_k)} - \sqrt{{\text{JS}}(F^{\calA}_k || F^{\calRO}_k)},
\end{align}
\end{defi}
The normalized average privacy leakage is further defined as
\begin{align*}
\epsilon_p^n = 2/(1+e^{-\epsilon_p}) - 1.
\end{align*} 

\textbf{Remark:} Note that $\epsilon_p^n\in [0,1]$, and $\epsilon_p^n = 1$ when $d(F^{\calA}_k || F^{\calRO}_k) = 0$.
\fi











\subsection{Applications of Privacy-Utility Trade-off}
%\XZ{should be Trade-Off?} 
\label{sec:application}
%\lipsum[8]

In this section, we apply the no free lunch theorem between the Bayesian privacy leakage and utility loss on three privacy-preserving mechanisms: Randomization \cite{geyer2017differentially,truex2020ldp,abadi2016deep}, Sparsity \cite{shokri2015privacy, gupta2018distributed, thapa2020splitfed}, and Homomorphic Encryption \cite{gentry2009fully,batchCryp}. We analyze the influence of specific protection mechanisms' parameters on the fluctuation of privacy leakage and utility loss.



\subsubsection{Randomization Mechanism}
\hfill

In SFL, one of the \textit{Randomization} methods is to add random noise such as Gaussian noise to model gradients \cite{abadi2016deep,geyer2017differentially,truex2020ldp}. Let $W_k^{\calRO} \in \mathcal W^{\calRO}_k$ be the parameter sampled from distribution $P_k^{\calRO} = \calN(\mu_0,\Sigma_0), k =1\cdots K$, where $\mu_0 \in \mathbb{R}^n$, $\Sigma_0 = \text{diag}(\sigma_{1}^2,\cdots, \sigma_{n}^2)$ is a diagonal matrix. Adding noise in the parameter could be expressed as $W_k^{\calD} = W_k^{\calRO} + \epsilon_k$, where $\epsilon_k \sim \calN(0, \Sigma_\epsilon)$ and $\Sigma_\epsilon = \text{diag}(\sigma_\epsilon^2, \cdots, \sigma_\epsilon^2)$. Therefore, $W_k^{\calD}$ follows the distribution $P_k^{\calD} = \calN(\mu_0, \Sigma_0+ \Sigma_\epsilon)$. The server aggregates all the protected parameters as $W_a^{\calD} = \frac{1}{K}\sum_{k=1}^K (W_k^{\calRO} + \epsilon_k)$ following the distribution $P^{\calD}_a = \calN(\mu_0, \Sigma_0/K+ \Sigma_\epsilon/K)$. The following theorem establishes bounds for the privacy leakage and utility loss using the variance of the noise $\sigma_\epsilon^2$ (see Appendix \ref{sec:proof-random-app} for the full proof).
%(please see the detailed relation in Proposition \ref{prop:random-sigma}).
%We take adding the Gaussian noise as an example to analyze. 
%In this setting, we have 

%\pref{thm: privacy-utility-tradeoff-random} 


%In this setting, the following theorem establishes the connection between the variance of adding Gaussian noise $\sigma_\epsilon$ and Bayesian privacy leakage \& utility loss of the federated system.

%For the randomization mechanism adding Gaussian noise, we illustrate the change of privacy leakage and utility loss with the change of variance of the Gaussian noise $\sigma_\epsilon^2$:

\begin{thm}\label{thm: privacy-utility-tradeoff-random} For the randomization mechanism by adding Gaussian noise, the privacy leakage and utility loss are bounded using variance of the Gaussian noise $\sigma_\epsilon^2$,

\begin{align} \label{tradeoff-random}
C_1
\leq \epsilon_{p} + \frac{C_3}{K}\min\left\{1,\sigma_\epsilon^2\sqrt{\sum_{i=1}^n\frac{1}{\sigma_{i}^4}}\right\},
\end{align}
and
\begin{align} \label{tradeoff-random-utility}
\epsilon_u \leq C_4 \min\left\{1,\sigma_\epsilon^2\sqrt{\sum_{i=1}^n\frac{1}{\sigma_{i}^4}}\right\},
\end{align}
where $C_1 = \frac{1}{K}\sum_{k=1}^K \sqrt{{\text{JS}}(F^{\calRO}_k || F^{\calO}_k)}, C_3 =(e^{2\xi}-1)/2$ are two constants independent of the protection mechanisms adopted, and $C_4$ is a constant satisfying that  $U(w,s)\leq C_4$ for any $w \in \mathcal{W}_k$ and $s \in \calS_k$.
\end{thm}


\textbf{Remark:} In this application, we assume $W_k^\calRO$ follows Gaussian distribution $\calN(\mu_0,\Sigma_0)$. In particular, when $\Sigma_0$ tends to zero, the Gaussian distribution degenerates into the one-point distribution when the algorithm converges. Moreover, the estimation of the variable $\gamma$ in \pref{thm: utility-privacy trade-off_JSD_mt} is shown in Appendix \ref{sec:proof-random-app}.

\begin{prop}%\HL{issues to fix} 
\label{prop:random-sigma}
If $\sigma_\epsilon^2\sqrt{\sum_{i=1}^n\frac{1}{\sigma_{i}^4}} \leq 1$, then we have
\begin{itemize}
\item The Bayesian privacy leakage $\epsilon_{p}$ is at least $C_1 - \frac{C_3}{K} \sigma_\epsilon^2\sqrt{\sum_{i=1}^n\frac{1}{\sigma_{i}^4}} $, which is a decreasing function of $\sigma_\epsilon$.
\item The utility loss $\epsilon_u$ is at most $C_4\sigma_\epsilon^2\sqrt{\sum_{i=1}^n\frac{1}{\sigma_{i}^4}}$, which is an increasing function of $\sigma_\epsilon$.
\end{itemize}
% \begin{itemize}
% \item The lower bound of the Bayesian privacy leakage $\epsilon_{p}$ is $C_1 - \frac{C_3}{K} \sigma_\epsilon^2\sqrt{\sum_{i=1}^n\frac{1}{\sigma_{i}^4}} $, which is a decreasing function of $\sigma_\epsilon$.
% \item The utility loss $\epsilon_u$ has the upper bound: $\sigma_\epsilon^2\sqrt{\sum_{i=1}^n\frac{1}{\sigma_{i}^4}}$, which is an increasing function of $\sigma_\epsilon$.
% \end{itemize}
% \begin{itemize}
% \item The Bayesian privacy leakage of federated system $\epsilon_{p}$ has the lower bound: $C_1 - \frac{C_3}{K} \sigma_\epsilon^2\sqrt{\sum_{i=1}^n\frac{1}{\sigma_{i}^4}} $, which is a decreasing function of $\sigma_\epsilon$.
% \item The utility loss $\epsilon_u$ has the upper bound: $\sigma_\epsilon^2\sqrt{\sum_{i=1}^n\frac{1}{\sigma_{i}^4}}$, which is an increasing function of $\sigma_\epsilon$.
% \end{itemize}
\end{prop}
Proposition \ref{prop:random-sigma} demonstrates that when the variance of adding noise $\sigma_\epsilon$ decreases, the lower bound of Bayesian privacy leakage $\epsilon_{p}$ increases. % as the variance of adding noise ($\sigma$) decreases. 
In particular, when $\sigma_\epsilon = 0$, $\sigma_\epsilon^2\sqrt{\sum_{i=1}^n\frac{1}{\sigma_{i}^4}} =0$.
Therefore, $ \epsilon_u=0$ and $\epsilon_{p} \geq C_1$. As a result, at least $C_1$ privacy leakage might be incurred due to the exposure of unprotected model information to adversaries who may launch Bayesian inference attacks. This theoretical analysis is in accordance with the empirical evidence demonstrated in \cite{zhu2020deep,he2019model}.


\subsubsection{Sparsity Mechanism}
\hfill

In SFL, clients launch the sparsity mechanism by uploading the partial parameters to the server. Specifically, each client uploads $d$ of total $n$ dimensions to the server. Let $W_k^{\calRO}\in \mathcal W^{\calRO}_k$ represent the parameter sampled from distribution $P^{\calRO}_k = \calN(\mu_0,\Sigma_0)$, where $\mu_0 = (\mu_u, \mu_o), \mu_u \in\mathbb R^d, \mu_o \in\mathbb R^{n-d}$ and $\Sigma_0 = \text{diag}(\Sigma_u^{d\times d}, \Sigma_o^{(n-d)\times (n-d)})$ is a diagonal matrix. Without loss of generality, we assume each client uploads the first $d$ dimensions to the server. We assume the vector composed by the last $(n-d)$ dimensions follows a Gaussian distribution denoted as $\calN(\mu_g, \Sigma_g)$, where $\Sigma_g$ is a diagonal matrix. In this setting, the protected model information follows $P_k^\calD \sim \calN(\mu, \sigma)$, where $\mu = (\mu_u, \mu_g), \Sigma = \text{diag}(\Sigma_u^{d\times d}, \Sigma_g^{(n-d)\times (n-d)})$. Then server aggregates all the uploaded parameters of clients as $W_a^{\calD}=\frac{1}{K}\sum_{k=1}^KW_k^\calD$ following the distribution $\calN(\mu,\Sigma/K)$, and $W_a^\calRO = \frac{1}{K}\sum_{k=1}^KW_k^\calRO$ follows the distribution $\calN(\mu_0,\Sigma_0/K)$. The following theorem illustrates bounds for privacy leakage and utility loss using the dimension of the uploaded model information $d$. The full proof is deferred to Appendix \ref{sec:proof-sparisty-app}.















% In SFL, clients launch the sparsity mechanism by uploading the partial parameters to the server. Specifically, they only upload $d$ of total $n$ parameters to the server. 

% Let $W_k^{\calRO}\in \mathcal W^{\calRO}_k$ be the parameter sampled from distribution $P^{\calRO}_k = \calN(\mu_0,\Sigma_0)$, where $\mu_0 = (\mu_u, \mu_o), \mu_u \in\mathbb R^d, \mu_o \in\mathbb R^{n-d}$ and $\Sigma_0 = diag(\Sigma_u^{d\times d}, \Sigma_o^{(n-d)\times (n-d)})$ is a diagonal matrix. Each client uploads their $d$ of total $n$ parameters with the same position. Without loss of generality, we assume the server uploads their first $d$ parameters to the server, that is, the distributions of first $d$ dimensions for variable $W_k^\calRO$ and $W_k^\calD$ are the same. Let $P_k^{\calD}$ be the distribution $\calN(\mu,\Sigma)$, where $\mu = (\mu_u, \mu_g)$, $\Sigma = diag(\Sigma_u^{d\times d}, \Sigma_g^{(n-d)\times (n-d)})$, $\mu_g, \Sigma_g$ are the constants of mean of variance of Gaussian distribution the server guess. Then server aggregates all the uploaded parameters of clients as $W_a^{\calD}=\frac{1}{K}\sum_{k=1}^KW_k^\calD$ following the distribution $\calN(\mu,\Sigma/K)$\footnote{We assume each clients uploads the model information with the same position (dimension), and suppose they have the same $W_k^\calRO$ and $W_k^{\calD}$.}, and $W_a^\calRO = \frac{1}{K}\sum_{k=1}^KW_k^\calRO$ follows the distribution $\calN(\mu_0,\Sigma_0/K)$. The following theorem illustrates the relations between privacy \& utility and the dimensions of uploaded model information $d$ (please see the details of relation in Proposition \ref{prop:sparsity-prop}). The full proof is deferred to Appendix \ref{sec:proof-sparisty-app}.

\begin{thm}  \label{thm: privacy-utility-tradeoff-sparsity}
For the sparsity mechanism by uploading partial information to the server, denote $h(\mu_1, \Sigma_1, \mu_2, \Sigma_2) =\left(1-\frac{\text{det}(\Sigma_1)^{1/4}\text{det}(\Sigma_2)^{1/4}}{\text{det}\left(\frac{\Sigma_1+\Sigma_2}{2}\right)^{1/2}}\exp\{-\frac{1}{8}(\mu_1-\mu_2)^T(\frac{\Sigma_1+\Sigma_2}{2})^{-1}(\mu_1-\mu_2)\}\right)^{1/2}$, we have

\begin{align}
C_1 \leq \epsilon_p + C_3\cdot h(\mu_o, \mu_g, \Sigma_o, \Sigma_g),
\end{align}
and
\begin{align}
    \epsilon_u \leq C\cdot h(\mu_o, \mu_g, \Sigma_o, \Sigma_g),
\end{align}
where $C_1 = \frac{1}{K}\sum_{k=1}^K \sqrt{{\text{JS}}(F^{\calRO}_k || F^{\calO}_k)}, C_3 =\frac{\sqrt{2}(e^{2\xi}-1)}{2}$ are two constants independent of the protection mechanisms adopted, and $C$ is a  constant satisfying that $\sqrt{2}U(w,s) \leq C$ for any $w \in \mathcal{W}_k$ and $s \in \calS_k$.
\end{thm}

% Specifically, $d$ is the variable of $h(\mu_o, \mu_g, \Sigma_o, \Sigma_g)$, where $\mu_o, \mu_g$ are vectors in $n-d$ dimensions representing the dimension of uploaded model information, $n$ is the total dimensions of model information. In particular, the dimension of $\mu_o, \mu_g, \Sigma_o, \Sigma_g$ would decrease as $d$ increases. \\

% Specifically, $d$ is the variable of $h(\mu_o, \mu_g, \Sigma_o, \Sigma_g)$, where $\mu_o, \mu_g$ are vectors in $n-d$ dimensions representing the dimension of uploaded model information, $n$ is the total dimensions of model information. In particular, the dimension of $\mu_o, \mu_g, \Sigma_o, \Sigma_g$ would decrease as $d$ increases. \\
%\textbf{Remark:} The estimation of one variable in \pref{thm: utility-privacy trade-off_JSD_mt}: $\gamma = \frac{\sum_{k=1}^K {\text{TV}}(P_k^{\calRO} || P^{\calD}_k)}{{\text{TV}}(P^{\calRO}_a || P^{\calD}_a )}$ is shown in appendix \ref{app: random}. Moreover, if the importance of each dimension of model information for model utility is different, we denote the weight matrix for model utility as $\alpha = (\alpha_1, \cdots, \alpha_n)$ for $n$ dimension of model information. The weight matrix $\alpha$ also influences utility loss. The upper bound of utility loss becomes large when the weight factor $\alpha_i$ increases, representing the upper bound of utility loss mainly depends on some important factors $\alpha_i$ with large value.

\begin{prop} \label{prop:sparsity-prop}
For the sparsity mechanism by uploading partial information to the server, we have: 
\begin{itemize}
    \item The Bayesian privacy leakage $\epsilon_{p}$ is at least $C_1 - C_3\cdot h(\mu_o, \mu_g, \Sigma_o, \Sigma_g)$, which is an increasing function of the dimension of uploaded model information $d$.
    \item The utility loss $\epsilon_u$ is at most $ C\cdot h(\mu_o, \mu_g, \Sigma_o, \Sigma_g)$, which is a decreasing function of the dimension of uploaded model information $d$.
\end{itemize}
\end{prop}

Proposition \ref{prop:sparsity-prop} demonstrates that when the dimension of uploaded model information $d$ increases, the lower bound of Bayesian privacy leakage $\epsilon_{p}$ increases, and the upper bound of utility loss $\epsilon_u$ decreases. In particular, $d= n$ implies that the server uploads all parameters to the server, then $ h(\mu_o, \mu_g, \Sigma_o, \Sigma_g)= 0$. Therefore, $\epsilon_p \geq C_1$ and $\epsilon_u = 0$. It shows that at least $C_1$ Bayesian privacy leakage occurs, but the utility is not sacrificed.



\subsubsection{Homomorphic Encryption} 
\hfill \\
Homomorphic Encryption (HE) \cite{gentry2009fully,rivest1978data,gentry2010toward} allows certain computation (e.g., addition) to be performed directly on ciphertexts, without decrypting them first. Such characteristic allows applying HE into FL to protect privacy because the server only accesses the uploaded parameters of users on ciphertexts instead of clients’ plaintext directly \cite{zhang2020batchcrypt,zhang2019pefl, aono2017privacy, truex2019hybrid}. Specifically, in federated learning, the uploaded model weights or gradients have been encrypted by the clients themselves. Therefore, it is hard for adversaries to espy the exposed information and infer clients' private data. The following theorem evaluates the privacy leakage and utility loss of the \textbf{approximate eigenvector} method \cite{gentry2013homomorphic}, which is a widely-used method of HE.

%demonstrates two widely-used methods of HE: \textbf{Paillier} \cite{paillier1999public} and \textbf{approximate eigenvector} method \cite{gentry2013homomorphic}.
%, where \textbf{approximate eigenvector} method is proved to be semantically secure \cite{regev2009lattices}. 




\begin{thm} \label{thm:tradeoff-HE}
For the encryption mechanism that encrypts the model information ($W_k^\calD = \text{Enc}(W_k^\calRO)$ using \textbf{approximate eigenvector} method), we firstly have 
\begin{equation}
\epsilon_{p} = 0.
\end{equation}
Furthermore, we have that
\begin{equation}
\epsilon_u \geq \frac{C_1}{C_2}.
\end{equation}
\end{thm}
\textbf{Remark:} For the encryption method, the Bayesian privacy leakage is zero because encryption satisfies semantic security, with which $S_k$ is independent of $W_k^{\calD}$. Moreover, utility loss has the lower bound $\frac{C_1}{C_2}$ because the private key of HE is unknown and the global model $\text{Enc}(W_a^{\calRO})$ remains encrypted to compute the utility loss.\\ 
\textbf{Remark:} In case that the HE private key is used by authorized users or is mistakenly disclosed to adversaries then the $\epsilon_p$ is also large although the utility loss might be small as well.














==> sections/05-discussion.tex <==
\section{Discussion}\label{sect:compare-BP}

The section illustrates the comparison of the proposed Bayesian Privacy with respect to Differential Privacy \cite{dwork2014algorithmic}, Bayesian Differential Privacy BDP \cite{BDP-icml20}, Local Differential Privacy \cite{duchi2013local} and Information Privacy \cite{du2012privacy}. A brief summary of the comparison is summarized in Table \ref{tab:tradeoff-comp}.


\begin{table}[htbp]
%\small
\footnotesize
\begin{tabular}{|c|c|c|c|c|}
\hline
& Def. 
%& \begin{tabular}[c]{@{}c@{}}Threat \\ models\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}Protection\\ mech.\end{tabular} &
\begin{tabular}[c]{@{}c@{}} Privacy-Utility\\Trade-off \end{tabular} &
%\begin{tabular}[c]{@{}c@{}}Prior\\ Depen.\end{tabular}
\begin{tabular}[c]{@{}c@{}}Applied \\ to FL \end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}} DP \cite{dwork2014algorithmic}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}$\frac{\Pr[M(S) \in W]}{\Pr[M(S')\in W]} \in [e^{-\epsilon},e^\epsilon]$\\ for any \textit{adjacent} data $S,S'$ \end{tabular} &\begin{tabular}[c]{@{}c@{}} Add noise \& \\ randomized response \end{tabular}& \begin{tabular}[c]{@{}c@{}} error $n \in \Omega(\frac{1}{\epsilon})$ 
\\ (Theo. 8.7 \cite{dwork2014algorithmic})\end{tabular} 
 & \cite{seif2020wireless,truex2020ldp} \\ \hline
\begin{tabular}[c]{@{}c@{}} LDP\cite{duchi2013local}\end{tabular} %,cormode2018privacy
&\begin{tabular}[c]{@{}c@{}} 
$\sup \Big\{\frac{Q(S|x)}{Q(S|x')}\Big\} \le \exp(\alpha)$
\\ for any data $x,x'$ \end{tabular} 
%&\begin{tabular}[c]{@{}c@{}}$\frac{\Pr[M(S) \in W]}{\Pr[M(S')\in W]} \in [e^{-\epsilon},e^\epsilon]$\\ for any data $S,S'$ \end{tabular} 
%& 
& \begin{tabular}[c]{@{}c@{}} Add noise \& \\ randomized response \end{tabular}
&\begin{tabular}[c]{@{}c@{}} $c_l\min\{1,\frac{1}{\sqrt{n\alpha^2}},\frac{d}{n\alpha^2} \}\le \mathfrak{M}_n $ \\ (Theo.1 \cite{duchi2013local}) \end{tabular}
& \begin{tabular}[c]{@{}c@{}} \cite{kim2021federated,truex2020ldp} \\ \cite{zhao2020local,seif2020wireless} \end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}} BDP \cite{BDP-icml20}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}$ \Pr \big[\log \frac{P(W|S)}{P(W|S')}\ge \epsilon_\mu \big]\le \delta_\mu$\\ for any \textit{adjacent} data $S,S'$ \\
differing by point $x' \sim \mu(x)$\end{tabular}
%&
& \begin{tabular}[c]{@{}c@{}} Add noise \& \\ randomized response \end{tabular} 
& N.A. 
&\cite{FL-BDP19} \\ \hline
% & $\mu(x)$ \\ \hline
\begin{tabular}[c]{@{}c@{}} IP \cite{du2012privacy}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}$\frac{p_{S|U}(s|u)}{p_{S}(s)} \in [e^{-\epsilon},e^\epsilon]$\\ for any $s$ and any $u$\end{tabular}
%&
&\begin{tabular}[c]{@{}c@{}} Add noise \\ (e.g., Laplacian) \end{tabular} 
&\begin{tabular}[c]{@{}c@{}}min IP s.t. distortion \\ (Def. 3 \cite{du2012privacy})\end{tabular} 
&no \\ \hline
\begin{tabular}[c]{@{}c@{}} Bayesian \\ Privacy \end{tabular} 
%\begin{tabular}[c]{@{}c@{}}Bayesian Privacy \\ with JS (BP)\end{tabular} 
& \begin{tabular}[c]{@{}c@{}} $\Big({JS(F^{\calA}_k || F^{\calO}_k)}\Big)^{\frac{1}{2}}\le \epsilon$, 
\\ for any threat model (Def. \ref{defi: average_privacy_JSD})
%and $ \frac{f_{S_k|W_k}(s|w)}{f_{S_k}(s)}\in [e^{-\delta}, e^{\delta}]$ 
\end{tabular} 
%& \begin{tabular}[c]{@{}c@{}}Bayesian Infer. \\Attack (Def. ?)\end{tabular} 
& 
\begin{tabular}[c]{@{}c@{}}Add noise, Sparsity \& \\ %\\Homomorphic Encryption 
HE (Sect.\ref{sec:application})\\ \end{tabular} 
& \begin{tabular}[c]{@{}c@{}}$ C_1 \le\epsilon_{p} + C_2\epsilon_{u}$ 
\\No free lunch theo. \end{tabular} 
& \begin{tabular}[c]{@{}c@{}} this \\ article \end{tabular}%\& \\ Sparsity 
\\ \hline
\end{tabular}
\caption{Comparison of privacy-utility trade-offs with Bayesian Privacy (BP) and related privacy measurements, namely, Diff. Privacy (DP) \cite{dwork2014algorithmic}, Local DP (LDP) \cite{duchi2013local}, Bayesian DP (BDP) \cite{BDP-icml20} and Information Privacy (IP) \cite{du2012privacy}. \label{tab:tradeoff-comp}}
\end{table}
%\XZ{$F_k^{\calB}$ represents the prior belief of the attacker, maybe it is not appropriate to say for any $\calB$.}

\subsection{The comparison with Differential Privacy and its variants}
\label{subsect:compare-BP-DP}
%\HL{Diff between BP and DP (BP/ DP could model dlg?), BP includes DP.}
%\textbf{Remark:}

We illustrate the comparison of Bayesian Privacy with respect to Differential Privacy and its variants as follows. 
\begin{itemize}
%\begin{enumerate}
\item First, the privacy-utility trade-off analyzed in differential privacy (DP) is essentially characterized by a reciprocal relation as shown by Theorem 8.7 of \cite{dwork2014algorithmic}, which dedicates that the outputs protected by an $\epsilon$-differentially private mechanism have the maximum error $\Omega\left(\frac{1}{\epsilon}\right)$. This trade-off analysis is in contrast to the \textit{No free lunch theorem} (\pref{thm: utility-privacy trade-off_JSD_mt}) in the present article, which dictates that the sum of privacy loss and utility loss is greater than a problem-dependent constant.

\item Second, it is shown that a $\xi$-maximum Bayesian privacy preserving mapping $f_{W|S}(\cdot)$ is $(2\xi)$-differentially private (see Appendix \ref{appendix:proof-BP-DP} for details). 
%We extend the analysis for quantifying the trade-off to the setting when privacy loss is measured using differential privacy. Combining \pref{lem: bp_to_dp} and \pref{property: TriangleiIneq}, we provide a quantitative relationship between privacy and utility for differential privacy.

% {
% \begin{lem}\label{lem: bp_to_dp}
% For any $\delta\ge 0$, let $f_{W|S}(\cdot)$ be a privacy preserving mapping that guarantees \textbf{$\delta$-maximum Bayesian privacy}. That is,
% \begin{align*}
% \frac{f_{S|W}(s|w)}{f_{S}(s)}\in [e^{-\delta}, e^{\delta}],
% \end{align*}
% for any $w\in\mathcal W$.
% Then, for any pair of parameters $w$ and $w'$, it holds that the mapping $f_{W|S}(\cdot)$ is $(2\delta)$-Differentially Private:
% \begin{align*}
% \frac{f_{S|W}(s|w)}{f_{S|W}(s|w')} \in [e^{-2\delta}, e^{2\delta}]. 
% \end{align*}
% \end{lem}
% \textbf{Discussion:} When $\delta = 0$, this definition requires that for any parameter $w$, the estimated distribution of the private information given $w$ is identical with that of the private information. Considering the optimal parameter $w^{\star}$, $\delta = 0$ implies that the estimated distribution of the private information given $w^{\star}$ is identical with that of the private information. It further implies that $w$ is independent of $s$.

% \begin{proof}
% From the definition of maximum privacy leakage, we know that
% \begin{align*}
% \frac{f_{S|W}(s|w)}{f_{S}}\in [e^{-\delta}, e^{\delta}],
% \end{align*}
% for any $w\in\mathcal W$.

% Therefore, for any $w, w'\in\mathcal W$ we have
% \begin{align*}
% \frac{f_{S|W}(s|w)}{f_{S|W}(s|w')} = \frac{f_{S|W}(s|w)}{f_{S}(s)}/\frac{f_{S|W}(s|w')}{f_{S}(s)}\in [e^{-2\delta}, e^{2\delta}]. 
% \end{align*}
% \end{proof}
% }

\item Third, the privacy-utility trade-off established by the local differential privacy dedicates that, for an $\alpha${-private} estimator, its \textit{minimax error bound} (in utility) is greater than a constant that is proportional to $\frac{1}{\alpha^2}$ (see Theorem 1 in \cite{duchi2013local}). 

\item Fourth, Bayesian Differential Privacy (BDP)  was also proposed to measure the privacy loss following Bayesian rule \cite{duchi2013local}. Nevertheless, BDP estimated the posterior of query outputs (denoted by $S$) given private data (denoted by $x$). This is in sharp contrast to the proposed Bayesian Privacy, which models adversaries' posterior belief of private data (denoted by $S$) given publicly exchanged information (denoted by $W^\calD$). Moreover, no privacy-utility trade-off analysis was provided for BDP in \cite{duchi2013local}. 

\item Last but not least, DP and its variants are not amenable to include encryption as a protection mechanism. To our best knowledge, the SFL framework based on Bayesian inference attack is the first that is applicable to different privacy-protection mechanisms, including both randomization in Differential Privacy \cite{geyer2017differentially,truex2020ldp,abadi2016deep} and Homomorphic Encryption \cite{gentry2009fully,batchCryp}. 

%\end{enumerate}
\end{itemize}

\subsection{The relationship between Bayesian Privacy and Information Privacy}\label{subsect:compare-BP-IP}

There are three fundamental differences between Bayesian Privacy (BP) and Information Privacy (IP) \cite{du2012privacy} as shown below. 
\begin{itemize}%{enumerate}
\item One fundamental difference between BP and IP lies in the fact that BP is formulated within a \textit{secure federated learning} setting as illustrated in Sect. \ref{sec:framework}, while it is unclear how to apply IP for delineating the privacy-utility trade-off in distributed learning scenarios. 

\item As per the privacy definitions, BP involves the \textit{averaged} gain of information about private data that an adversary may obtain by observing publicly exposed model information (see Def. \ref{defi: average_privacy_JSD} in this article). On the other hand, information privacy is defined based on the \textit{bound} of such information gain (see Def. 6 in \cite{du2012privacy}). 
Note that we also give the bounds of Bayesian Privacy in Eq. (\ref{eq:ep-bayes-privacy}), which is nevertheless based on the average gain. 

\item In terms of the privacy-utility trade-off, the optimal trade-off in BP is cast as the solution of a constrained optimization where the goal is to minimize utility loss subject to the hard constrain of maintaining Bayesian privacy leakage less than an acceptable threshold (the problem in Eq. (\ref{eq: key_constraint_upper_bound})). In contrast, the optimal trade-off in IP is to minimize the privacy leakage subject to a given utility loss constrain (Def. 3 in \cite{du2012privacy}). 

\end{itemize}%{enumerate}



==> sections/06-conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

%Question: Does the generalized JS metric satisfy triangle inequality?

%Inspired by the concept of semantic security, 
In this article, we proposed a statistical framework in SFL based on Bayesian inference attack to take into account two compelling requirements i.e. the protection of private data as well as the maximization of model utility in secure federated learning (SFL). The proposed framework is based on the cornerstone definition of Bayesian privacy Leakage that quantitatively measures the amount of information about private data that semi-honest adversaries may infer from the espied information during the SFL learning process. %Technically, the BPL is measured by the distances between distributions of adversaries' \textit{prior} and \textit{posterior} beliefs about private data.
Then the trade-off privacy and utility is %then rigorously analyzed and is regarded 
formulated as an optimization problem in which the goal is to find a modified distribution of exchanged model information that achieves the smallest utility loss without incurring privacy loss above an acceptable level. The theoretical analysis of the trade-off then leads us to the No Free Lunch (NFL) theorem for federated learning, which dictates that one has to trade a high privacy persevering guarantee with a certain degree of utility loss, and vice versa. This trade-off analysis is applicable to two %three 
protection mechanisms including Randomization \cite{geyer2017differentially,truex2020ldp,abadi2016deep}
%, Sparsity \cite{shokri2015privacy, gupta2018distributed, thapa2020splitfed} 
and Homomorphic Encryption \cite{gentry2009fully,batchCryp} which are special cases of the general theorem proved in \pref{thm: utility-privacy trade-off_JSD_mt}. 
%It was shown that one cannot reduce both privacy loss and utility loss to zero. 

The analysis of privacy-utility trade-off in secure federated learning (SFL), to our best knowledge, is the first work that takes into account different specific protection mechanisms, including DP and HE, in a unified framework. While the main result disclosed in this article is inspiring, we plan to apply the technique we developed during this research endeavor to explore in the future the trade-off between efficiency and privacy, which itself is an active research topic for secure federated learning adopting Homomorphic Encryption to protect privacy. \\

%is measured using the divergence between the prior and posterior beliefs. We first define the global optimal parameters as the set of parameters that are optimal in terms of both privacy and utility. The optimal privacy parameters are the set of parameters that are optimal in terms of privacy leakage, considering the tolerance extent of the client. The optimal utility parameters are the set of parameters that are optimal in terms of utility loss. We aim at quantifying the trade-off between privacy leakage and utility loss for the scenarios containing global optimal parameters. 
%We provide lower bounds for the objective function, when privacy loss is measured using Jensen-Shannon divergence, $\alpha$-skew Jensen-Shannon divergence, and total variation distance. 
%We further analyze the widely-used protection mechanisms under our framework, including randomization mechanism, ...
